SQuALITY: Building a Long-Document Summarization Dataset the Hard Way

Summarization datasets are often assembled either by scraping naturally occurring public-domain summaries -- which are nearly always in difficult-to-work-with technical domains -- or by using approximate heuristics to extract them from everyday text -- which frequently yields unfaithful summaries. In this work, we turn to a slower but more straightforward approach to developing summarization benchmark data: We hire highly-qualified contractors to read stories and write original summaries from scratch. To amortize reading time, we collect five summaries per document, with the first giving an overview and the subsequent four addressing specific questions. We use this protocol to collect SQuALITY, a dataset of question-focused summaries built on the same public-domain short stories as the multiple-choice dataset QuALITY (Pang et al., 2021). Experiments with state-of-the-art summarization systems show that our dataset is challenging and that existing automatic evaluation metrics are weak indicators of quality.

==> tables/multiref-correlations.tex <==
\begin{table}[t]
    \centering
    \begin{tabularx}{\columnwidth}{lrrr} % right align numbers in table...
    \toprule
    metric & model only & human only & all \\
    \midrule
    ROUGE-1 & -7.4 & 6.8  & 63.1$^*$ \\
    ROUGE-2 & -7.8 & 5.2  & 42.8$^*$ \\
    ROUGE-L & -3.2 & 14.0 & 47.8$^*$ \\
    METEOR  & -11.1& -4.3 & 54.1$^*$ \\
    BERTScore & & & \\
    \bottomrule
    \end{tabularx}
    \caption{Pearson correlation between various automatic evaluation metrics and human judgments of overall quality. 
    Correlations are near zero and not statistically significant when only considering model-generated summaries ('model only') or only human-written summaries ('human only'). 
    Correlations are significantly positive when considering human- and model-written summaries together ('all').
    } % statistical significance
    \label{tab:correlations}
\end{table}


==> tables/question-templates.tex <==
\begin{table*}[t]
    \centering
    \begin{tabularx}{\textwidth}{X}
    \toprule
    What is the plot of the story? \\
    What happens to [character X] throughout the story? \\
    What is the relationship between [character X] and [character Y]? \\
    What is the setting of the story? \\
    What is the significance of [object X] on the rest of the story? \\
    How is [theme X] explored throughout the story? \\
    Story-specific questions \\
    %\midrule
    \bottomrule
    \end{tabularx}
    \caption{Question templates provided to writers. The question "What is the plot of the story?" is always answered by the writers. For more subjective templates such as "What is the significance of [object X]?" or "How is [theme X] explored?", we ask the writers to use these templates only in cases where they believe the answer is fairly straightforward and obvious.}
    \label{tab:question_templates}
\end{table*}

